Prospects of Gravitational Wave Follow-up Through a Wide-field Ultra-violet Satellite: a Dorado Case Study

The detection of gravitational waves from binary neuron star merger GW170817 and electromagnetic counterparts GRB170817 and AT2017gfo kick-started the field of gravitational wave multimessenger astronomy. The optically red to near infra-red emission (`red' component) of AT2017gfo was readily explained as produced by the decay of newly created nuclei produced by rapid neutron capture (a kilonova). However, the ultra-violet to optically blue emission (`blue' component) that was dominant at early times (up to 1.5 days) received no consensus regarding its driving physics. Among many explanations, two leading contenders are kilonova radiation from a lanthanide-poor ejecta component or shock interaction (cocoon emission). In this work, we simulate AT2017gfo-like light curves and perform a Bayesian analysis to study whether an ultra-violet satellite capable of rapid gravitational wave follow-up, could distinguish between physical processes driving the early `blue' component. We find that a Dorado-like ultra-violet satellite, with a 50 sq. deg. field of view and a limiting magnitude (AB) of 20.5 for a 10 minute exposure is able to distinguish radiation components up to at least 160 Mpc if data collection starts within 3.2 or 5.2 hours for two possible AT2017gfo-like light curve scenarios. We also study the degree to which parameters can be constrained with the obtained photometry. We find that, while ultra-violet data alone constrains parameters governing the outer ejecta properties, the combination of both ground-based optical and space-based ultra-violet data allows for tight constraints for all but one parameter of the kilonova model up to 160 Mpc. These results imply that an ultra-violet mission like Dorado would provide unique insights into the early evolution of the post-merger system and its driving emission physics.

==> GW follow-up with Dorado/acronyms.tex <==

\begin{acronym}
\acro{1D}{one dimensional}
\acro{2D}{two dimensional}
\acro{3D}{three dimensional}
\acro{BH}{black hole}
\acro{BHNS}{black hole neutron star}
\acro{BBH}{binary black hole}
\acro{BNS}{binary neutron star}
\acro{CBC}{compact object coalescence}
\acro{CCD}{charge coupled device}
\acro{DETC}{Dorado exposure time calculator}
\acro{DOS}{Dorado observation scheduler}
\acro{EFE}{Einstein field equations}
\acro{effwav}[$\lambda_\mathrm{eff}$]{effective wavelength}
\acro{EM}{electromagnetic}
\acro{EoS}{equation of state}
\acro{ETC}{exposure time calculator}
\acro{FoV}{field of view}
\acrodefplural{FoV}{fields of view}
\acro{GCN}{$\gamma$-ray Coordinates Network}
\acro{GRMHD}{general-relativistic magneto-hydrodynamic}
\acro{GRB}{$\gamma$-ray burst}
\acro{GW}{gravitational wave}
\acro{GWB}{gravitational wave background}
\acro{HLV}{Advanced LIGO and Virgo}
\acro{HLVK}{Advanced LIGO, Virgo and KAGRA}
\acro{HPDI}{highest posterior density interval}
\acro{IR}{infra-red}
\acro{ISM}{interstellar medium}
\acro{LIGO}{Laser Interferometer Gravitational-Wave Observatory}
\acro{LCO}{Las Cumbres Observatory}
\acro{lumdist}[$d_L$]{luminosity distance}
\acrodefplural{lumdist}[$d_L$]{luminosity distances}
\acro{LVC}{LIGO-Virgo collaboration}
\acro{MMA}{multi-messenger astronomy}
\acro{NIR}{near infra-red}
\acro{NS}{neutron star}
\acro{PPD}{posterior probability distribution}
\acrodefplural{PPD}{posterior probability distributions}
\acro{S/N}{signal-to-noise ratio}
\acro{SDSS}{Sloan Digital Sky Survey}
\acro{SED}{spectral energy density}
\acrodefplural{SED}{spectral energy densities}
\acro{sGRB}{short $\gamma$-ray burst}
\acro{SED}{spectral energy distribution}
\acro{ToO}{target of opportunity}
\acrodefplural{ToO}{targets of opportunity}
\acro{UV}{ultra-violet}
\acro{UVO}{\ac{UV} and optical}
%\acro{UVOIR}{ultra-violet/ optical/ infra-red}
\acro{UVOIR}{\ac{UV}, optical and \ac{IR}}
\end{acronym}

==> GW follow-up with Dorado/shorthands.tex <==
\def\bfa{Bayes factor}
\def\bfs{Bayes factors}
\def\blue{\ac{UV} and optically blue}
\def\Bright{`Lower early opacity'}
\def\distances{\ac{lumdist} = \SI{40}{Mpc}, \SI{100}{Mpc} and \SI{160}{Mpc}}
\def\D{\textit{Dorado}}
\def\distone{\SI{40}{\mega\parsec}}
\def\disttwo{\SI{100}{\mega\parsec}}
\def\default{`default'}
\def\bright{`lower early opacity'}
\def\data{photometric data}
\def\Default{`Default'}
\def\gbo{ground-based optical}
\def\gw{GW170817}
\def\gfo{AT2017gfo}
\def\grb{GRB170817A}
\def\kn{kilonova}
\def\knmodel{kilonova model}
\def\knmodels{kilonova models}
\def\pipeline{full light curve simulation pipeline}
\def\red{optically red and \ac{NIR}}
\def\sbu{satellite-based \ac{UV}}
\def\sh{shock interaction}
\def\shmodel{shock interaction  model}
\def\shmodels{shock interaction  models}
\def\Shmodel{Shock interaction  model}





